Kishu: Time-Traveling for Computational Notebooks

Computational notebooks (e.g., Jupyter, Google Colab) are widely used by data scientists. A key feature of notebooks is the interactive computing model of iteratively executing cells (i.e., a set of statements) and observing the result (e.g., model or plot). Unfortunately, existing notebook systems do not offer time-traveling to past states: when the user executes a cell, the notebook session state consisting of user-defined variables can be irreversibly modified - e.g., the user cannot 'un-drop' a dataframe column. This is because, unlike DBMS, existing notebook systems do not keep track of the session state. Existing techniques for checkpointing and restoring session states, such as OS-level memory snapshot or application-level session dump, are insufficient: checkpointing can incur prohibitive storage costs and may fail, while restoration can only be inefficiently performed from scratch by fully loading checkpoint files. In this paper, we introduce a new notebook system, Kishu, that offers time-traveling to and from arbitrary notebook states using an efficient and fault-tolerant incremental checkpoint and checkout mechanism. Kishu creates incremental checkpoints that are small and correctly preserve complex inter-variable dependencies at a novel Co-variable granularity. Then, to return to a previous state, Kishu accurately identifies the state difference between the current and target states to perform incremental checkout at sub-second latency with minimal data loading. Kishu is compatible with 146 object classes from popular data science libraries (e.g., Ray, Spark, PyTorch), and reduces checkpoint size and checkout time by up to 4.55x and 9.02x, respectively, on a variety of notebooks.

==> sections/data/restore_undo_table_backup.tex <==
notebook criu dump en criuinc ours

1 1.202 1.704 0.1670 5.603 0.160
2 0.681 1.842 0.1365 1.591 0.1350
3 10.040 8.0100 2.200 16.341 0.021
4 0.7630 2.059 0.377 1.873 0.073
5 2.162 2.1927 2.274 6.205 0.404
6 1.068 2.013 1.836 3.219 0.128
7 0.9300 1.172 0.4281 5.561 0.1555
8 0.727 1.016 0.3304 3.740 0.1366
9 6.208 4.827 1.204 14.333 0.244
10 7.523 4.814 1.352 13.617 0.588
11 0 1.8299 1.1283 0 0.2390
12 0 1.7020 0.1279 0 0.0853

13 0 1.8299 1.1283 0 0.2390
14 0 1.7020 0.1279 0 0.0853

15 0.966 0 2.037 08.127 0.2166



==> sections/data/restore_undo_table_backup_2.tex <==
notebook criu dump en criuinc ours

1 1.202 1.704 0.1670 5.603 0.160


2 2.162 2.1927 2.274 6.205 0.404

3 0.9300 1.172 0.4281 5.561 0.1555


4 7.523 4.814 1.352 13.617 0.588

5 0.966 0 2.037 8.127 0.2166
6 0 1.8299 1.1283 0 0.2390





==> sections/problem_setup.tex <==
\section{Efficient Incremental Checkpointing}
\label{sec:data_modeling}

\subfile{plots/symbols_table}

This section describes \system's data modeling for achieving time-traveling between notebook session states.
We formally define the Application History Graph for modeling the lineage of a single session state in \cref{sec:data_modeling_ahg_def} and its construction in \cref{sec:data_modeling_ahg_construct}. Then, we define the Checkpoint Graph for modeling relations between multiple session states in \cref{sec:problem_setup_cgraph_def} and its construction in \cref{sec:data_modeling_cgraph_construct}.

% which models the lineage of a notebook session for efficient session state replication. \Cref{tbl:symbols} lists a summary of the notations we use in this section. 
% We provide a formal definition of the AHG in \Cref{sec:ahg_graph} and describe how the AHG enables exact session state replication in \cref{sec:ahg_problem}.

% In this section, we formalize \system's notebook session lineage modeling and describe \system's optimization problem of picking the most efficient C/R configuration.
% \Cref{tbl:symbols} lists a summary of the notations we use in this section.
% \Cref{sec:dependency_graph} describes \system's dependency graph.
% \Cref{sec:problem_definition} defines the optimization problem of session C/R.


\subsection{Application History Graph}
\label{sec:data_modeling_ahg_def}

The AHG is a directed acyclic graph expressing how a session state has changed with respect to cell executions. \cref{fig:problem_setup_graph} is an example.

\paragraph{Preliminary: Variables vs. Objects}
In Python, variables and objects are 2 distinct concepts: A \textbf{variable} is a named entity (e.g., \texttt{df}) from which one or more \textbf{object} (which can be uniquely identified by its object ID) are reachable - for example, for a list, each of the elements is an (possibly non-unique) object.
The set of all objects reachable from any variable (i.e., \textsc{X}) defined in the global namespace forms the session state.

\begin{definition}
    A \textbf{Variable Blob} is a set of variable names from which the reachable objects form a \textbf{connected component}.
\end{definition}

A variable blob can consist of one variable name (e.g., a primitive, \texttt{x = 1}) or multiple variable names from which the same object can be reached (i.e., shared references, \texttt{(x, y)} is a variable blob if \texttt{id(x.foo) = id(y[0])}. An example is given in \textcolor{red}{figure}.
The variable blob is the granularity level at which we record accesses and updates in the AHG: that is, cell executions may modify the objects referenced from variables in the same variable blob with or without changing the (1) variable names or (2) membership of the blob (i.e., through disconnecting references), as follows:

\begin{definition}
    A \textbf{Variable Blob Snapshot} (VBS) is a nameset-timestamp pair $((x_1,...,x_i), t)$ representing the variable blob $(x_1,...,x_i)$ created/modified (i.e., updated) at timestamp $t$. We denote the set of VBSes as $\mathcal{V}$.
\end{definition}

\begin{definition}
    A \textbf{Cell Execution} (CE) $c_t$ represents a cell execution that finishes at timestamp $t$.
\end{definition}

Cell executions are \textit{linear}; that is, for each session, there is at most one cell running at a time, and their cell executions are totally ordered. We denote the list of CEs by $\mathcal{C}$.

\begin{definition}
    A \textbf{write dependency} $c_{t} \rightarrow ((x_1,...,x_i), t)$
        indicates 
        CE $c_{t}$ may have modified/created (i.e., updated) at time $t$ (1) the object(s) reachable from a variable name $x_j, 1 \leq j \leq i$ in the variable blob $((x_1,...,x_i), s)$.
    We denote the set of write dependencies as $\mathcal{E}_w$.
\end{definition}
In \cref{fig:problem_setup_graph}, 
$c_{t_3}$ modifies \texttt{x} with ``\texttt{x += 1}''; hence, ($c_{t_3}$ $\rightarrow$ (\texttt{x}, $c_{t_3}$)).
Modifications can also be \textit{membership changes}: for example, $c_{t_4}$ disconnects \texttt{y} from \texttt{z} with ``\texttt{y.foo = None}''; hence, there is both ($c_{t_4}$ $\rightarrow$ (\texttt{y}, $c_{t_4}$)) and ($c_{t_4}$ $\rightarrow$ (\texttt{z}, $c_{t_4}$)), even though objects reachable from \texttt{y} were not explicitly modified by $c_{t_4}$.

\begin{definition}
    A \textbf{read dependency} $((x_1,...,x_i), s) \rightarrow c_{t}$
        indicates CE $c_{t}$ has accessed object(s) reachable from a variable name $x_j, 1 \leq j \leq i$ in the variable blob $((x_1,...,x_i), s)$
        last created/modified at time $s$.
        % where (some reachable object of) \texttt{x} was last created/modified at time $s$ and is expressed by a directed edge
        % from VS $(x, s)$ to CE $c_{t}$:
    We denote 
    the set of read dependencies by $\mathcal{E}_r$.
\end{definition}

\noindent
In \cref{fig:problem_setup_graph}, 
``\texttt{print(y.foo)}'' in $C_{t_2}$ accesses a field in the object \texttt{y} - hence, the variable blob \texttt{(y, z)} (even though \texttt{z} was not explicitly accessed) after the blob's creation in $c_{t_1}$; hence there is ((\texttt{y}, \texttt{z}), $c_{t_1}$) $\rightarrow$ $c_{t_2}$.
%

\begin{definition}
    The \textbf{AHG} $G := \{\mathcal{V}\cup\mathcal{C}, \, \mathcal{E}_w\cup \mathcal{E}_r\}$ is a bipartite graph,
        where $\mathcal{V}$ is VSes, $\mathcal{C}$ is CEs;
            $\mathcal{E}_w$ and $\mathcal{E}_r$ are write/read dependencies, respectively.
    % its bipartition of nodes are the VSs and CEs, while its edges are the read and write dependencies. 
    It models the lineage of the notebook session.
\end{definition}

\noindent
In sum, the AHG formalizes accesses/modifications to the session state with respect to cell executions at the Variable Blob level (i.e., level of connected components of objects).
It also helps \system reason about what objects currently exist in the sessions state via \textit{Active VBSes}, as follows:

\begin{definition}
    VBS $((x_1,...,x_i), t_i)$ is \textbf{active} if 
        $(x_1,...,x_i)$ is in the namespace (i.e., not deleted), and 
        there is no VBS $((x_1,...,x_i), t_j)$ such that $t_i < t_j$.
\end{definition}

\noindent
An active VBS $((x_1,...,x_i), t_i)$ represents the current version of the Variable Blob $(x_1,...,x_i)$.
% the version of $x$ at checkpoint time (i.e., the most up-to-date version). 
For example, for the session state after executing $c_{t_5}$ (in \cref{fig:problem_setup_graph}), 
``(\texttt{x}, $t_3$)'' is active since \texttt{x} was last modified by $c_{t_3}$. 
We denote the set of active VBSes as $\mathcal{V}_a$.

\paragraph{Why Variable Blob-Level Granularity?}
Defining accesses and modifications to the session state at the Variable Blob level serves multiple benefits. First, it helps bind the size of the AHG to scale linearly with the number of connected components of objects, which is typically far less than the total number of underlying objects (which can be very large for lists and dataframes).
Second, It aids \system in correctly preserving variable aliases and shared references that form the basis of Variable Blobs: this is because if we mix data recomputation and loading for different variable names in the same variable blob, we risk breaking the shared reference~\cite{lielasticnotebook}.
Finally, variable blobs help us reason mathematically in a much cleaner fashion when determining the versioning of objects in the session state for incremental checkpointing (\textcolor{red}{cref}) and checkout (\textcolor{red}{cref}).
% \paragraph{Variable Blob Snapshot}
% \begin{itemize}
%     \item A connected component of objects
%     \item Minimal granularity of items in KV store
%     \item Multiple variables which share object references identified via ID graph (cite ElasticNotebook)
%     \item Versioned: has timestamp corresponding to time of last cell execution that modified it
%     \item Why we need blobs?\begin{itemize}
%         \item Correctly preserve variable aliases/shared references
%         \item Cite ElasticNotebook: mix recomputation and data loading for variable blobs, shared references are broken
%         \item Much cleaner in terms of mathematical model
%     \end{itemize}
% \end{itemize}

% \paragraph{Cell Execution}
% Timestamped.
% \paragraph{Application History Graph}
% Bipartitie graph between variable blob snapshots and Cell Executions.

\subsection{Incremental AHG Construction}
\label{sec:data_modeling_ahg_construct}
We describe how \system constructs the AHG accurately.

\paragraph{Constructing the AHG} The AHG is incrementally built with 
accessed/updated variable blobs by each cell execution: 
\begin{itemize}
    \item A new CE $c_t$ is created; $t$ is an execution completion time.
    \item Read dependencies are created from VBSes $((x_{1_1},...,x_{1_i}), t_{x_1})$, ..., $((x_{k_1},...,x_{k_i}), t_{x_k})$ to $c_t$, where $(x_{1_1},...,x_{1_i}),...,(x_{k_1},...,x_{k_i})$ are variables blobs accessed by $c_t$.
        % and each variable was last modified by CEs $c_{t_{x_1}},...,c_{t_{x_k}}, t_{x_1},...,t_{x_k} < t$ prior to execution.
    \item VSes $(y_{1_1},...,y_{1_i}), t)$, ..., $(y_{k_1},...,y_{k_i}), t)$ are created for variable blobs $(y_{1_1},...,y_{1_i}),...,(y_{k_1},...,y_{k_i})$ \emph{possibly} updated by $c_t$. 
    Write dependencies are added from $c_t$ to each of the new VBSes.
\end{itemize}
%
\cref{fig:problem_setup_graph} (right) shows an example AHG.
Identifying access/modified variable blobs is crucial for its construction,
which we describe below.

\paragraph{ID Graph}
The ID graph is a graph structure constructed following the pickle protocol~\cite{pickle} and represents the objects reachable from each variable name in the global namespace.
The ID graph captures shared references (e.g., aliases) and inter-variable relationships~\cite{lielasticnotebook} and is used to both (1) determine the membership of Variable Blobs (i.e., which objects are reachable from multiple variable names) and (2) detect updates to Variable Blobs.

\paragraph{Identifying Accessed Variables Blobs}
Accessed Variable Blobs are identified through results from the Patched Namespace \textcolor{red}{todo: figure}.
Since \system's Patched Namespace acts as the global namespace of the notebook session, it is impossible for the user to access variable names from within the notebook without being detected by \system;
Hence, \system's approach detects variable blob accesses with almost 100\% accuracy~\footnote{It is still possible for the user to access variables through unintended means, such as direct memory address accesses; however, we limit the scope of our work to normal notebook usage.}

\paragraph{Identifying Updated Variable Blobs}
\system Identifies updates to Variable Blobs through the ID graph.
After each cell execution, the current Variable Blobs' ID graphs are compared to the ones created before to capture (1) modifications to reachable objects and (2) Variable Blob membership changes.
Due to the implementation of the Pickle Protocol, \system's update detection is \textit{conservative}: that is, it may result in \textit{false positives} if objects are dynamically generated (e.g., datatype objects) with a different memory address each time during the construction of the ID graph (i.e., traversal).
However, it will never result in false negatives (\textcolor{red}{experiment})

% \begin{itemize}
%     \item If any name in a variable blob is modified, the entire blob is modified. E.g., {x, y, z} is a blob, x is modified -> {x, y, z} is modified
%     \item Conservative modification detection. E.g., {x, y, z} is a blob, z points to x and y; z no longer points to x and y next cell execution, but the blob {x, y} is still modified.
% \end{itemize}

\paragraph{Optimized Update Detection}
\system achieves optimized Variable Blob update detection with the help of the Patched Namespace: only Variable Blobs that have member names that were either accessed (\texttt{\_\_getitem\_\_}) or assigned to (\texttt{\_\_setitem\_\_}) can be candidates for updates, hence we can greatly speed up the update detection process if we only have to check a small portion of the variable names (hence Variable Blobs) in the namespace after each cell execution. We empirically verify the time savings achieved by this approach in (\textcolor{red}{experiment}).
% \begin{itemize}
%     \item By using variable blob as granularity, only variables that were touched in the patched namespace (and variables linked to touched variables) can be candidates for modification, speeding up modification detection
%     \item Short proof: modifying a variables requires using the name directly (detected) or using an alias (detected via links). Assigning the name to an alias will also be detected.
% \end{itemize}
\subsection{Checkpoint Graph Formal Definition}
\label{sec:problem_setup_cgraph_def}

The Checkpoint Graph is a directed tree of checkpoints (\textcolor{red}{todo: figure}), defined as follows:

\begin{definition}
    A \textbf{Checkpoint} is a (saved) session state directly following a cell execution and is represented by a unique ID $\alpha_i$.
\end{definition}
As \system (incrementally) saves the session state following each cell execution, there are as many checkpoints $\alpha_i$ in the Checkpoint Graph as there are cell executions.
We denote the set of checkpoints as $\mathcal{A}$.

\paragraph{Contents of Each Checkpoint}
Each checkpoint $\alpha_i$ is associated with two items (\cref{sec:system_workflow}): (1) an AHG $\mathcal{G}_{\alpha_i}$ representing the lineage of cell executions up to the time of the checkpoint, and (2) some stored active VBSes (determined by a checkpoint plan, \textcolor{red}{cref}) which form part of the session state at the time of the checkpoint.

\begin{definition}
    A \textbf{parent-child relation} $\alpha_i \rightarrow \alpha_j$ exists between two \textbf{Checkpoints} $\alpha_i$ and $\alpha_j$ if the state of $\alpha_j$ can be obtained from the state of $\alpha_i$ by performing one cell execution - specifically, the one made directly prior to $\alpha_j$.
\end{definition}

The parent-child relations form the edges of the Checkpoint Graph, and the branches are the exploration paths.
Notably, for parent-child pair $\alpha_i \rightarrow \alpha_j$, the AHG $\mathcal{G}_{\alpha_i}$ of commit $\alpha_i$ is contained within the AHG $\mathcal{G}_{\alpha_j}$ of commit $\alpha_j$; specifically, $\mathcal{G}_{\alpha_j}$ contains exactly one more cell execution $c_{t_j}$ compared to $\mathcal{G}_{\alpha_i}$, and executing $c_{t_j}$ in the state of $\alpha_i$ results in the state of $\alpha_j$.

\begin{definition}
    A \textbf{Branch} $\alpha_{i_1},...,\alpha_{i_k}$ is a directed path in the Checkpoint Graph consisting of multiple parent-child relations: $\alpha_{i_1} \rightarrow \alpha_{i_2},...,\alpha_{i_{k-1}} \rightarrow \alpha_{i_k}$. It represents a series of states that can be obtained by performing a series of cell executions in succession.
\end{definition}

There can be multiple (diverging) branches in the Checkpoint Graph resulting from checkouts (\cref{sec:data_modeling_cgraph_construct}).
From these branches, we can define the notion of \textit{ancestor} and \textit{lowest common ancestor}, as follows:

\begin{definition}
    A Checkpoint $\alpha_i$ is an \textbf{ancestor} of $\alpha_j$ there exists a Branch $...,\alpha_i,...,\alpha_j$ containing both $\alpha_i$ and $\alpha_j$, with $\alpha_j$ occurring after $\alpha_i$. This means that $\alpha_j$ can be obtained from $\alpha_i$ through a series of cell (re-)executions.
\end{definition}

\begin{definition}
    A Checkpoint $\alpha_k$ is \textbf{lowest common ancestor} of $\alpha_i$ and $\alpha_j$ if $\alpha_k$ is an ancestor of both $\alpha_i$ and $\alpha_j$, and there is no other checkpoint $\alpha_{k'}$ that $\alpha_k$ is an ancestor of with this property. That is, lowest common ancestors represent the point of where branches diverge.
\end{definition}

Due to the total ordering implied by ancestor relations, if an active VBS $((x_1,...,x_k), t_{\alpha_i})$ is stored in checkpoint $\alpha_i$ and active VBS with the same membership differing by timestamp only $((x_1,...,x_k), t_{\alpha_j})$ is stored in checkpoint $\alpha_j$, and $\alpha_i$ is an ancestor of $\alpha_j$, then the timestamps $t_{\alpha_i} < t_{\alpha_j}$.
That is, the session state of $\alpha_j$ must be newer than that of its ancestor $\alpha_i$.
Ancestor and lowest common ancestor relations are used to reason about which intermediate data (based on versioning principles) we can utilize when creating checkpoints and performing checkout, which we describe in detail in \textcolor{red}{cref} and \textcolor{red}{cref}.

% \begin{itemize}
%     \item An AHG: \begin{itemize}
%         \item Represents lineage of cell executions up to the point of the commit
%         \item AHG has as many cell execution nodes as the commit has ancestors
%     \end{itemize}
%     \item Variable Blob Snapshots stored from that commit:\begin{itemize}
%         \item Each VBS is associated with a commit - the VBS at a timestamp specific to that commit.
%     \end{itemize}

% \end{itemize}

% \paragraph{Formal Definition}
% Directed tree of checkpoints:\begin{itemize}
%     \item Each checkpoint assigned unique ID and represents a session state
%     \item checkpoint a is ancestor of b -> b can be reached from a via a series of cell executions
%     \item checkpoint c is lowest common ancestor of a and b -> both a and b can be reached from c, with no c’ reachable from c sharing the same property
% \end{itemize}

\subsection{Checkpoint Graph Construction}
\label{sec:data_modeling_cgraph_construct}
The incremental construction of the Checkpoint Graph is analogous to Git Versioning. It requires the notion of a head checkpoint, defined as follows:
\begin{definition}
    The \textbf{head checkpoint} in the Checkpoint Graph is a checkpoint representing the current session state. It is updated when new checkpoints are created (from performing cell executions), and when checkout is performed.
\end{definition}
The head checkpoint of the Checkpoint Graph is analogous to the HEAD of Git versioning~\cite{commitgraph}.
We depict a summary in \textcolor{red}{figure}.

\paragraph{Creating a New Checkpoint}
When a new checkpoint is created, a new node (i.e., checkpoint) $\alpha_j$ is created under the current head checkpoint $\alpha_i$, and a parent-child relation $\alpha_i \rightarrow \alpha_j$ is added. 
This effectively extends the branch which previously had the head checkpoint $\alpha_i$ as the leaf node by one node $\alpha_j$.

\paragraph{Performing a Checkout}
When a checkout is performed to return to a previous checkpoint $\alpha_k$, the head is moved to $\alpha_k$. If $\alpha_k$ has existing children (e.g., $\alpha_{k+1}$), then the next checkpoint $\alpha_{l}$ will be placed in a new branch --- $\alpha_k$ will be the lowest common ancestor of $\alpha_{k+1}$ and $\alpha_{l}$.

% \begin{itemize}
%     \item Analogus to Git Versioning
%     \item Creating a new checkpoint: follow same branch, create child under HEAD
%     \item Checking out: Go back to commit to check out, next commit will be placed in a new branch
% \end{itemize}
